Mixture Encoder for Joint Speech Separation and Recognition

Multi-speaker automatic speech recognition (ASR) is crucial for many real-world applications, but it requires dedicated modeling techniques. Existing approaches can be divided into modular and end-to-end methods. Modular approaches separate speakers and recognize each of them with a single-speaker ASR system. End-to-end models process overlapped speech directly in a single, powerful neural network. This work proposes a middle-ground approach that leverages explicit speech separation similarly to the modular approach but also incorporates mixture speech information directly into the ASR module in order to mitigate the propagation of errors made by the speech separator. We also explore a way to exchange cross-speaker context information through a layer that combines information of the individual speakers. Our system is optimized through separate and joint training stages and achieves a relative improvement of 7% in word error rate over a purely modular setup on the SMS-WSJ task.

==> tables/results_context.tex <==

\begin{table}[htbp]

\centering
\caption{Using soft cross-speaker context}
\label{table:results_context}
\begin{tabular}{|c|c|c|}
\hline
\multirow{2}{*}{Soft Context} & \multicolumn{2}{c|}{WER [\%]} \\\cline{2-3}
    & dev'93 & eval'92 \\\hline
 no &   19.8 &    14.0 \\\hline
yes &      ? &       ? \\
\hline
\end{tabular}

\end{table}


==> tables/results_literature.tex <==

\begin{table}[htbp]
        \centering
        \caption{Comparison of results reported in the literature for the clean WSJ and SMS-WSJ corpora. \#Ch denotes the number of microphone channels used.}
        \label{table:results_literature}
        \setlength{\tabcolsep}{3.5pt}
        \begin{tabular}{|c|c|c|S|S|}
                \hline
                \multirow{2}{*}{Corpus} & \multirow{2}{*}{Model}   & \multirow{2}{*}{\#Ch} & \multicolumn{2}{c|}{WER [\%]}           \\\cline{4-5}
                                        &                          &                            & {dev'93}                      & {eval'92} \\\hline\hline
                clean WSJ               & LF-MMI \cite{hadian2018LFMMI}   & \multirow{2}{*}{-}         & {-}                           & 2.9     \\\cline{2-2}\cline{4-5}
                                        & ours                     &                            & 5.4                           & 3.0     \\\hline
                SMS-WSJ                 & Joint Sep. \& ASR \cite{zhang2022joint}    & 6                          & {-}                           & 15.4    \\\cline{2-5}
                                        & 2-spkr ASR \cite{zhang2022joint}    & \multirow{5}{*}{1}         & {-}                           & 35.0    \\\cline{2-2}\cline{4-5}
                                        & U-Net TCN \cite{wang2021multi}     &                            & {-}                           & 28.7    \\\cline{2-2}\cline{4-5}
                                        & SepFormer \cite{cord2022monauralSep} &                          & {-}                           & 26.5    \\\cline{2-2}\cline{4-5}
                                        & TF-GridNet \cite{wang2022tfGridNet} &                            & {-}                           & 7.9     \\\cline{2-2}\cline{4-5}
                                        & ours                     &                            & 19.1                          & 13.6    \\
                \hline
        \end{tabular}

\end{table}


==> tables/results_modular.tex <==

\begin{table}[htbp]

\centering
\caption{Modular \gls{AM} (separated signals are treated independent of each other)}
\label{table:results_modular}
\begin{tabular}{|c|c|c|c|}
\hline
\multirow{2}{*}{\# Params} & \multirow{2}{*}{Joint Training} & \multicolumn{2}{c|}{WER [\%]} \\\cline{3-4}
                     &     & dev'93 & eval'92 \\\hline
\multirow{2}{*}{51M} &  no &   21.7 & 15.6 \\\cline{2-4}
                     & yes &   20.4 & 14.6 \\\hline
\multirow{2}{*}{80M} &  no &   23.1 & 16.7 \\\cline{2-4}
                     & yes &   20.8 & 14.9 \\
\hline
\end{tabular}
% Note: results are not final

\end{table}

